Modular Valenced Temperley-Lieb Algebras

We investigate the representation theory of the valenced Temperley-Lieb algebras in mixed characteristic. These algebras, as described in characteristic zero by Flores and Peltola, arise naturally in statistical physics and conformal field theory and are a natural deformation of normal Temperley-Lieb algebras. In general characteristic, they encode the fusion rules for the category of $U_q(\mathfrak{sl}_2)$ tilting modules. We use the cellular properties of the Temperley-Lieb algebras to determine those of the valenced Temperley-Lieb algebras. Our approach is, at heart, entirely diagrammatic and we calculate cell indices, module dimensions and indecomposable modules for a wide class of valenced Temperley-Lieb algebras. We present a general framework for finding bases of cell modules and a formula for their dimensions.

==> questions.tex <==
\section{Questions to Answer}

When we study the representation theory of algebras, we typically have a hierarchy of questions we want to know the answers to.  These are adapted from Barcelo and Ram's excellent survey on the subject~\cite{barcelo_ram_1997}.
\begin{enumerate}[(Q1)]
  \item What is the dimension of the algebra?
  \item How many finitely generated, simple modules does it have?
  \item Can we index the simple modules?
  \item What is the dimension of the simple modules?
  \item How do we construct the simple modules?
  \item What are the indecomposable modules?
  \item What are the composition factors of the indecomposable modules?
  \item What are the structures of their composition series?
\end{enumerate}
When we know the algebra is cellular, we have an alternative set of tasks (typically we will know the involution already).
\begin{enumerate}[(CQ1)]
  \item What is the set $\Lambda$?
  \item What are the sets of tableaux $M(\lambda)$?
  \item What is the set $\Lambda_0$?
  \item What are the composition multiplicities of simple modules in cell modules (decomposition numbers)?
\end{enumerate}
These are related by
\begin{align*}
  \text{CQ1} + \text{CQ2}                                            & \Rightarrow \text{Q1}\\
  \text{CQ3}                                                         & \Rightarrow \text{Q2} + \text{Q3} + \text{Q5} + \text{Q6}\\
  \text{CQ1} + \text{CQ2} +\text{CQ3} + \text{\cref{lem:folklore_1}} & \Rightarrow \text{Q4}\\
  \text{CQ4}                                                         & \Rightarrow \text{Q7}
\end{align*}

